Topological structure of complex predictions

Complex prediction models such as deep learning are the output from fitting machine learning, neural networks, or AI models to a set of training data. These are now standard tools in science. A key challenge with the current generation of models is that they are highly parameterized, which makes describing and interpreting the prediction strategies difficult. We use topological data analysis to transform these complex prediction models into pictures representing a topological view. The result is a map of the predictions that enables inspection. The methods scale up to large datasets across different domains and enable us to detect labeling errors in training data, understand generalization in image classification, and inspect predictions of likely pathogenic mutations in the BRCA1 gene.

==> details.tex <==
\subsection{Details of ImageNet experiment}
\paragraph{Dataset construction}
\paragraph{Model and parameters}

% For figure~\ref{highlight_15_with_images}, we pick a group of 4 or 9 images that connected in the graph we show. We embed these images in a grid on top of the graph. The center of the grid is computed as the mean coordinates of the grid of images. We pick image groups manually that appear far enough from each other on the visualization so that we can avoid overlap of images and cover as many local structures on the visualization as possible.
\subsection{Details of gene mutation experiment}
\paragraph{Dataset construction} We download gene variants experiments from the official ClinVar website~\cite{landrum2018clinvar}. We choose all experiments that are targeting \textbf{BRCA1} as it is one of the genes with the most number of experiments and part of the protein it encodes has known 3D structures. Gene variants without a valid VCF (variant call format) position are removed. For each gene variant, we follow the same steps as proposed by~\cite{avsec2021effective} to compute its embedding. First, we extract the reference and alternate DNA sequences from homo sapiens (human) genome assembly, either hg19 or hg38 as specified by the gene variant record. That is, a 393,216bp long DNA sequence with the VCF position as center is extracted. Note that for the alternate sequence, the gene variant is applied first before extracting the modified sequence. Then, we direclty use the pretrained model from~\cite{avsec2021effective} to make predicitons on the reference and alternate sequences. This model will aggregate the centering 114,688bp into 128-bp bins of length 896. The prediction for each 128bp bin is a 5,313 vector, where each element represents the predicted gene expression in one of the 5,313 genome tracks for the human genome (including 2,131 transcription factor chromatin immunoprecipitation and sequencing tracks, 1,860 histone modification tracks, 684 DNase-seq or ATAC-seq tracks and 638 CAGE tracks). The prediction vector of the 4 128bp bins located in the center is then sum together to get a prediction vector for the reference or alternate sequence. After that, the elements in each prediction vector corresponding to the CAGE tracks is $log(1+x)$ transformed. Finally, we compute the difference of preprocessed prediciton vectors between reference and alternate sequences as the final embedding for the gene variant. In total, we get a 23,376-by-5,313 embedding matrix for 23,376 gene variant records. As for the labels, We directly use the ``ClinSigSimple'' field as the label of each gene variant record. An integer 1 means at least one current record indicates ``Likely pathogenic'' or ``Pathogenic'', but doesn't necessarily mean this record includes assertion criteria or evidence. An integer 0 means no current record of ``Likely pathogenic'' or ``Pathogenic''. An integer -1 means no clinic significance and is replaced by label 0 in our experiments. 
\paragraph{Model and parameters} The embedding matrix for 23,376 gene variants is first standardized along each column, then randomly splitted into 50\% training and 50\% testing. A logistic regression model is trained on the training data with $\ell_1$ penalty to be 1. To build the graph, the embedding matrix is PCA reduced to 128 with PCA whitening and then each row is $\ell_2$ normalized. A 5-NN graph is constructed on the preprocessed embedding matrix with cosine similarity. We use 2 prediction lens and the first 2 PCA lens of the embedding matrix for GTDA analysis. The splitting threshold, overlapping ratio, the smallest node size and the smallest component size is set to be 30, 5\%, 5 and 5 respectively.
\subsection{Details of running time analysis}
\paragraph{Machine and parameters} All running time are reported on a server with 4 AMD EPYC 7532 processors (128 cores in total) and 504 GB memory. For Amazon Products, we tested a few sets of parameters and chose $K=1000$, $s_1=40$, $s_2=10$, $r=0.1\%$ as this set of parameters can build a reeb graph whose maximum component size is below 2000 so that a simple layout algorithm can be applied. We also tested $K=2000, 500$, $s_1=10,20$, $r=0.5\%$ and the running time is very similar for the other sets of parameters. For the other datasets, we simply report running time using the same parameters as described in the corresponding experiment section. The running time includes all steps as described in algorithm~\ref{GTDA}.

==> figures_low_res/mutation/stats.tex <==
\begin{table}[tp]
\tiny 
\centering
%\arrayrulecolor{lightgray}
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
& \multicolumn{4}{c}{Prediction and Type (coding regions of 1JNX)} & & \multicolumn{4}{c}{Prediction and Type (all)} & \\
\cmidrule{2-5} 
\cmidrule{7-10}
& Harmful & Harmful & non-Harm & non-Harm & \shortstack{Chi-square \\p-value} & Harmful & Harmful & non-Harm & non-Harm & \shortstack{Chi-square \\p-value}\\
\cmidrule(lr){2-3} 
\cmidrule(lr){4-5} 
\cmidrule(lr){7-8} 
\cmidrule(lr){9-10}
Component & SNV & non-SNV & SNV & non-SNV &  & SNV & non-SNV & SNV & non-SNV  \\
\midrule
0&11&6&83&4&5.1e-04&13&6&167&8&1.2e-04\\ \arrayrulecolor{lightgray} \hline
2&0&0&0&0&-&17&264&49&16&1.2e-36\\ \hline 
3&1&3&99&5&1.8e-05&12&3&230&9&2.5e-02\\ \hline 
4&0&0&0&0&-&13&14&181&4&1.2e-16\\ \hline 
6&0&10&10&2&-&24&38&298&20&2.7e-27\\ \hline 
7&0&0&0&0&-&6&42&152&24&1.5e-22\\ \hline 
8&0&4&0&0&-&16&82&96&22&6.2e-21\\ \hline 
9&0&0&0&0&-&6&23&44&11&4.9e-07\\\hline 
10&0&0&0&0&-&17&102&129&22&1.0e-30\\ \hline 
14&0&2&2&0&-&13&31&297&19&7.6e-30\\ \hline 
15&6&2&40&0&-&25&146&437&24&8.7e-90\\ \hline 
16&0&0&0&0&-&6&155&136&13&3.9e-53\\ \hline 
17&5&14&49&4&6.5e-08&55&93&485&23&2.7e-59\\ \hline 
18&0&0&2&0&-&9&7&115&3&7.5e-08\\ \hline 
19&0&8&0&2&-&36&70&422&32&1.0e-44\\ \hline 
21&0&6&64&2&-&20&31&376&17&4.7e-33\\ \hline 
22&12&16&102&2&4.2e-13&32&20&188&6&1.1e-12\\ \hline 
25&0&0&0&0&-&15&17&19&3&7.7e-03\\ \hline 
26&0&0&0&0&-&34&4&256&12&2.4e-01\\ \hline 
28&0&1&0&1&-&29&42&63&12&1.7e-07\\ \hline 
29&3&6&193&18&8.1e-07&9&9&339&31&1.3e-07\\ \hline 
30&0&0&0&0&-&19&57&93&9&6.4e-19\\ \hline 
31&0&0&0&0&-&16&18&68&8&4.3e-06\\ \hline 
32&0&4&2&0&-&5&23&51&5&1.0e-10\\ \hline 
33&10&55&64&11&5.5e-16&16&55&204&23&1.1e-28\\ \hline 
34&16&18&32&0&-&32&70&66&12&3.5e-12\\ \hline 
36&2&4&250&6&1.8e-12&8&11&314&23&3.2e-12\\ \hline 
37&0&0&0&0&-&40&76&26&14&1.5e-03\\ \hline 
38&0&0&0&0&-&21&37&137&19&8.6e-14\\ \hline 
39&0&0&0&0&-&14&198&24&14&3.4e-18\\ \hline 
40&0&2&6&0&-&50&81&488&13&1.5e-63\\ \hline 
41&0&0&2&0&-&16&14&158&6&1.1e-11\\ \hline 
44&0&0&0&0&-&27&29&423&17&4.2e-30\\ \hline 
46&0&16&30&2&-&19&36&51&10&2.0e-07\\ \hline 
48&0&4&20&4&-&30&14&220&16&3.1e-06\\ \hline 
50&0&0&62&0&-&4&36&262&10&2.2e-45\\ \hline 
52&0&4&18&2&-&60&67&830&79&5.7e-40\\ \hline 
53&0&0&0&0&-&15&27&303&25&2.7e-22\\ \hline 
54&0&0&10&0&-&19&27&365&13&2.5e-32\\ \hline 
55&0&0&0&0&-&21&19&109&3&2.8e-11\\ \hline 
56&0&0&0&0&-&5&34&29&4&9.4e-10\\ \hline 
57&0&0&0&0&-&40&18&78&6&4.5e-04\\ \hline 
58&2&2&0&0&-&25&30&157&10&2.3e-15\\ \hline 
59&0&0&0&0&-&17&44&163&6&6.6e-28\\ \hline 
60&6&0&36&2&-&6&7&130&13&2.8e-05\\ \hline 
62&2&33&12&7&1.9e-05&12&69&218&35&8.1e-33\\ \hline 
64&2&25&114&7&5.0e-22&6&25&192&17&4.4e-22\\ \hline 
66&0&4&24&0&-&27&23&165&9&1.9e-12\\ \hline 
67&0&6&0&0&-&9&30&111&4&1.0e-20\\ \hline 
68&21&13&87&9&3.3e-04&76&108&570&92&3.8e-36\\ \hline 
69&2&3&78&7&4.4e-03&4&11&314&35&8.6e-12\\ \hline 
70&0&0&0&0&-&40&48&6&6&1.0e+00\\ \hline 
71&0&0&0&0&-&17&8&269&18&4.4e-05\\ \hline 
72&0&0&12&0&-&6&5&318&21&1.7e-05\\ \hline 
73&0&0&0&0&-&12&9&142&3&3.1e-10\\ \hline 
74&0&0&0&0&-&19&11&119&15&1.5e-03\\ \hline 
77&6&20&14&4&1.1e-03&13&33&213&11&6.0e-28\\ \hline 
78&0&0&2&0&-&3&8&181&6&4.1e-16\\ \hline 
79&10&4&52&0&-&33&10&203&6&3.3e-06\\ \hline 
81&0&0&0&0&-&9&57&95&15&9.5e-21\\ \hline 
82&0&0&0&0&-&8&4&212&6&1.5e-05\\ \hline 
85&0&1&38&1&-&14&61&496&29&5.3e-65\\ \hline 
88&0&0&0&0&-&3&34&269&16&6.8e-41\\ \hline 
90&2&4&76&2&4.4e-07&10&4&162&4&1.0e-04\\ \hline 
99&0&0&8&0&-&6&3&100&7&3.3e-02\\ \hline 
100&0&0&2&0&-&4&6&64&34&2.2e-01\\ \hline 
101&0&2&2&0&-&6&4&60&6&2.8e-02\\ \hline 
102&0&0&0&0&-&7&9&109&5&5.3e-09\\ \hline 
Overall&148&344&2114&122&2.9e-259&1506&3986&16208&1338&0.0e+00\\
\arrayrulecolor{black}
\bottomrule
\end{tabular}
\caption{For each component in the Reeb networks, 2 contingency tables are computed, where the left table only considers variants in the coding regions of 1JNX and the right table considers all variants. Only components where each cell of the right table has a count 3 or higher are included. Chi-square p-values are computed for tables where each cell has a count larger than 0.}
\label{contigency}
\end{table}
